The Evolution of Binaries under the Influence of Radiation-Driven Winds from a Stellar Companion

Interacting binaries are of general interest as laboratories for investigating the physics of accretion, which gives rise to the bulk of high-energy radiation in the Galaxy. They allow us to probe stellar evolution processes that cannot be studied in single stars. Understanding the orbital evolution of binaries is essential in order to model the formation of compact binaries. Here we focus our attention on studying orbital evolution driven by angular momentum loss through stellar winds in massive binaries. We run a suite of hydrodynamical simulations of binary stars hosting one mass losing star with varying wind velocity, mass ratio, wind velocity profile and adiabatic index, and compare our results to analytic estimates for drag and angular momentum loss. We find that, at leading order, orbital evolution is determined by the wind velocity and the binary mass ratio. Small ratios of wind to orbital velocities and large accreting companion masses result in high angular momentum loss and a shrinking of the orbit. For wider binaries and binaries hosting lighter mass-capturing companions, the wind mass-loss becomes more symmetric, which results in a widening of the orbit. We present a simple analytic formula that can accurately account for angular momentum losses and changes in the orbit, which depends on the wind velocity and mass ratio. As an example of our formalism, we compare the effects of tides and winds in driving the orbital evolution of high mass X-ray binaries, focusing on Vela X-1 and Cygnus X-1 as examples.

==> preamble.tex <==
\usepackage{graphicx}
\usepackage{braket}
%\usepackage{amsmath}
\usepackage[utf8]{inputenc}
\usepackage [greek,british]{babel}
\usepackage [autostyle, english = american]{csquotes}
\MakeOuterQuote{"}
\newenvironment{rcases}
  {\left.\begin{aligned}}
  {\end{aligned}\right\rbrace}
  
  \usepackage[OT2,T1]{fontenc}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{floatflt}
%\usepackage[explicit]{titlesec}
\usepackage{wrapfig}
\usepackage[table,xcdraw,svgnames]{xcolor}
\usepackage{tabu}
\usepackage{appendix}
\usepackage{afterpage}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}

\usepackage[colorlinks]{hyperref} %

\newcommand{\pder}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\no{\noindent}
% Ecrire sa thèse en Français
% http://www.theses.ulaval.ca/wiki/index.php?title=Latex:R%C3%A9daction_en_fran%C3%A7ais

%\usepackage[T2A,T1]{fontenc}
%\usepackage{newpxtext,newpxmath}
\usepackage{newtxtext,newtxmath}
\usepackage{icomma}
\usepackage{microtype}
\usepackage[font=small,labelfont=bf]{caption}

%\usepackage{ae}
%\usepackage{aeguill}
%\usepackage{fancyhdr}
%\usepackage{subfig}
\usepackage{pdfpages}
\usepackage{url}
\usepackage{verbatim}
\usepackage{comment}
\usepackage{ulem}
\usepackage{color}
\usepackage{xspace}
%\usepackage{hyperref}
\usepackage{floatrow}
\usepackage{geometry}
\usepackage{rotating}
\usepackage{wallpaper}
  \usepackage{eso-pic}
\setlength{\headheight}{15pt} 
% Mise en page
\usepackage[rightcaption]{sidecap}
%\newcommand{\noMinitocPlease}{true}
%\usepackage{fancyhdr}
\ifx\noMinitocPlease\undefined
\usepackage{minitoc}
\mtcselectlanguage{british}
\else
\usepackage{mtcoff}
\fi

%\DeclareUnicodeCharacter{00A0}{ }

\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

%\usepackage{braket}

\usepackage{a4wide} 
%\usepackage{vmargin}
%\setmarginsrb{2cm}{1cm}{2cm}{1cm}{1cm}{1cm}{1cm}{1cm}
%\def\clearpage{\hspace{1cm}}
\usepackage{version}

%\usepackage[final]{pdfpages}
% \includepdf[pages=1-20]{fichier.pdf}

%% entete Audrey
%\usepackage[cyr]{aeguill}
%\usepackage{float} 
\usepackage{caption}

%----------------------------------------------------------------------------
%macro pour activer ou desactiver l'incrementation de la table des matières
%---------------------------------------------------
\makeatletter
\let\original@addcontentsline\addcontentsline
\newcommand{\dummy@addcontentsline}[3]{}
\newcommand{\DeactivateToc}{\let\addcontentsline\dummy@addcontentsline}
\newcommand{\ActivateToc}{\let\addcontentsline\original@addcontentsline}
\makeatother


%----------------------------------------------------------------------------
%mise en page
%----------------------------------------------------------------------------
\usepackage{fancyhdr}
\pagestyle{fancy}

%----------------------------------------------------------------------------
%en tête du haut
%----------------------------------------------------------------------------
\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\chaptermark}[1]{\markboth{\chaptername~\thechapter{} : #1}{}}
\renewcommand{\sectionmark}[1]{\markright{\thesection{} \ #1}}
\renewcommand{\sectionmark}[1]{\markright{\thesubsection{} \ #1}}
\lhead[]{\textsl{\rightmark}}
\rhead[\textsl{\leftmark}]{}

%----------------------------------------------------------------------------
%en tête du bas
%----------------------------------------------------------------------------
%\renewcommand{\footrulewidth}{1pt}
\fancyfoot[C]{\thepage} 

%----------------------------------------------------------------------------
% dédicace
%----------------------------------------------------------------------------
%\usepackage{multicol}
%\usepackage[linktocpage]{hyperref}
\usepackage{epigraph}
\newcommand{\dedicace}[1]{{%
\clearpage
\pagestyle{empty}
\setlength{\beforeepigraphskip}{10\baselineskip}
\setlength{\epigraphrule}{0pt}
%\epigraphtextposition{flushright}
\mbox{}
\epigraph{\itshape #1}{}}}

%----------------------------------------------------------------------------
% épigraphe
%----------------------------------------------------------------------------
\newcommand{\epigraphe}[2]{{%
\clearpage
\pagestyle{empty}
\setlength{\beforeepigraphskip}{10\baselineskip}
\mbox{}\epigraph{#1}{#2}}}

\newpage
\makeindex
%\renewcommand{\sc}{\textsc}
%\renewcommand{\bf}{\textbf}
%\renewcommand{\comment}[1]{({\textit *** #1 ***})}
\newcommand{\mathnotation}[2]{\newcommand{#1}{\ensuremath{#2}\xspace}}
\newcommand{\caca}[1]{\sout{#1}}
\renewcommand{\caca}[1]{}
\newcommand{\todo}[1]{\textcolor{red}{#1}}
%\renewcommand{\todo}[1]{#1}
\newcommand{\com}[1]{\textcolor{red}{(!!! #1 !!!)}}
\renewcommand{\com}[1]{}
\newcommand{\bof}[1]{\uwave{#1}}
\renewcommand{\bof}[1]{#1}
\newcommand{\xja}[1]{\uwave{#1}}
\renewcommand{\xja}[1]{#1}

\renewcommand{\epsilon}{\varepsilon}

%% Math notations ------------------------

\mathnotation{\mt}{m_t^* \xspace}
\mathnotation{\ml}{m_l^* \xspace}

\mathnotation{\VGone}{V_{g1}}
\mathnotation{\VGtwo}{V_{g2}}
\mathnotation{\Vback}{V_{bg}}
\mathnotation{\MUs}{\mu_{F,s}}
\mathnotation{\MUd}{\mu_{F,d}}

\mathnotation{\VGi}{{V_\mathrm{g \mathit{i}}}}
\mathnotation{\DVGi}{V_{\mathrm{g} \mathit{i}}^{\mathrm{AC}}}
\mathnotation{\DVGone}{V_{\mathrm{g} 1}^{\mathrm{AC}}}
\mathnotation{\DVGtwo}{V_{\mathrm{g} 2}^{\mathrm{AC}}}
\mathnotation{\VGonedc}{{V_{\mathrm{g1}}^{\mathrm{DC}}}}
\mathnotation{\VGtwodc}{{V_{\mathrm{g2}}^{\mathrm{DC}}}}
\newcommand{\VGidc}{$V_{\mathrm{g \mathit{i}}}^{\mathrm{DC}}$}
\newcommand{\Gin}{\Gamma_{\mathrm{in}}}
\newcommand{\vg[1]}{$V_{\mathrm{g#1}}$}
\newcommand{\diff[2]}{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\mathnotation{\ECM}{U'}
\newcommand{\DPHI}{$\varphi$}

\newcommand{\Pone}{P$\mathrm{_1}$}
\newcommand{\Ptwo}{P$\mathrm{_2}$}
\newcommand{\VG}{\ensuremath{V_g}\xspace}
\newcommand{\VD}{\ensuremath{V_d}\xspace}
\newcommand{\VBG}{$V\mathrm{_{bg}}$}
\newcommand{\IDS}{\ensuremath{I_{ds}}\xspace}
\mathnotation{\ION}{I_\text{on}}
\mathnotation{\IOFF}{I_\text{off}}
\newcommand{\GS}{\ensuremath{\Gamma_{\mathrm{S}}}\xspace}
\newcommand{\GD}{\ensuremath{\Gamma_{\mathrm{D}}}\xspace}
\newcommand{\GL}{\ensuremath{\Gamma_{\mathrm{L}}}\xspace}
\newcommand{\GR}{\ensuremath{\Gamma_{\mathrm{R}}}\xspace}
\newcommand{\GIN}{\ensuremath{\Gamma_{\mathrm{in}}}\xspace}
\newcommand{\GDEUX}{\ensuremath{\Gamma_{\mathrm{2}}'}\xspace}
\mathnotation{\CT}{\Delta}
\mathnotation{\AT}{\mathcal{T}}
\newcommand{\epsun}{\ensuremath{\epsilon_1}\xspace}
\newcommand{\epsdeux}{\ensuremath{\epsilon_2}\xspace}

\newcommand{\EConetwo}{$E_{C12}$}
\newcommand{\ZIMP}{z$_{\mathrm{imp}}$}

\mathnotation{\Do}{\mathrm{D}^0 \xspace}
\mathnotation{\Dion}{\mathrm{D}^+ \xspace}
\mathnotation{\Ddouble}{\mathrm{D}^- \xspace}

\mathnotation{\Restime}{R' \xspace}

\mathnotation{\GDR}{\Gamma_{2,R} \xspace}
\mathnotation{\GDL}{\Gamma_{2,L} \xspace}
\mathnotation{\GDS}{\Gamma_{2,S} \xspace}
\mathnotation{\GDD}{\Gamma_{2,D} \xspace}
\mathnotation{\TD}{T_{2,R} \xspace}
\mathnotation{\trie}{{\mathrm{e}^-}}
\mathnotation{\trih}{{\mathrm{h}^+}}

\mathnotation{\sigz}{\hat{\sigma}_z \xspace}
\mathnotation{\sigx}{\hat{\sigma}_x \xspace}
\mathnotation{\Bzero}{{\vec{B}}_0 \xspace}

\newcommand{\quantum}{\ensuremath{e^2/h}}

\usepackage[squaren,Gray]{SIunits}

\usepackage{blindtext}
\usepackage{enumitem}
\usepackage{xcolor}

\usepackage{aasmacros}
\usepackage{apacite}
\usepackage{natbib}
\setcitestyle{aysep={}} 
%\usepackage{breakcites}
%\usepackage{cite}

\def\d{{\mathrm d}}
%\newcommand{\degree}{\ensuremath{^\circ}}
%% --------------------------------------

\usepackage{silence}

\WarningFilter{minitoc(hints)}{W0023}
\WarningFilter{minitoc(hints)}{W0028}
\WarningFilter{minitoc(hints)}{W0030}
\WarningFilter{minitoc(hints)}{W0024}

% \usepackage{longtable}
\setlength{\parskip}{0pt}
\usepackage{indentfirst}
\usepackage{subfig}

\AtBeginDocument{%
\hypersetup{
  %colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = Maroon, %Colour of internal links
  citecolor   = blue, %Colour of citations
}}

